Good-case Early-Stopping Latency of Synchronous Byzantine Reliable Broadcast: The Deterministic Case (Extended Version)

This paper considers the good-case latency of Byzantine Reliable Broadcast (BRB), i.e., the time taken by correct processes to deliver a message when the initial sender is correct. This time plays a crucial role in the performance of practical distributed systems. Although significant strides have been made in recent years on this question, progress has mainly focused on either asynchronous or randomized algorithms. By contrast, the good-case latency of deterministic synchronous BRB under a majority of Byzantine faults has been little studied. In particular, it was not known whether a goodcase latency below the worst-case bound of t + 1 rounds could be obtained. This work answers this open question positively and proposes a deterministic synchronous Byzantine reliable broadcast that achieves a good-case latency of max(2, t + 3 -- c) rounds, where t is the upper bound on the number of Byzantine processes and c the number of effectively correct processes.

==> alg/sync-sig-brb-francois-V3.tex <==
\SetKwProg{InitStep}{Init:}{}{end~init}
\SetKwProg{ForAll}{for all}{ do}{end}
\SetKwProg{ForEach}{for each}{ do}{end}
\SetKwProg{InEachSynchroRound}{In each synchronous round}{ do}{end~round}
\SetKwProg{InSynchroRound}{In synchronous round}{ do}{end~round}
\SetKwProg{Fn}{Function}{ is}{end~function}

\SetKwIF{If}{ElseIf}{Else}{if}{then}{elseif}{else}{end~if}

\SetKwComment{Comment}{$\rhd$}{}
\SetCommentSty{textit}

\newcommand{\announceStep}[1]{%
  \medskip%
      
  {\SetKwComment{Comment}{}{}\Comment{\fbox{#1}}}
  \smallskip%
}

\begin{algorithm}[tb]
  \small
  \InSynchroRound{$R=1$}{
    %% \medskip
    %% \Comment{\fbox{Communication step}}\smallskip
    \broadcast $\msgm(\{m\cryptchain p_{\orig}\})$\label{line:porig:bcast}\;
    %% \medskip
    %% \Comment{\fbox{Delivery step}}%\smallskip
    $\brbdeliver(m)$\label{line:porig:brdeliver}\;
  }
  \caption{\brb-broadcast operation executed by $p_{\orig}$ }
  %when $R=1$} 
  \label{alg:porig:code}
\end{algorithm}

\begin{algorithm}[ht]
  \small
  \InitStep{}{
    %    $\view_i \leftarrow \{\}$ \;
    $\view_i \leftarrow [\emptyset, ..., \emptyset]$\label{line:viewi:modif}\Comment*{Array of size $\finalround$ containing the chains observed by $p_i$ in each round}
    $\ready_i \leftarrow \ffalse$ ;
    $\toBeBcast_{i,1} \leftarrow \emptyset$\;
    %% \lIf(\Comment*[f]{$p_i$ is the process that rb\_broacasts}){$p_i=p_\orig$}{
    %%   $\toBeBcast_{i,1} \leftarrow \{m_\orig\cryptchain p_\orig\}$%\Comment*{$m_\orig$ is the message $p_\orig$ is rb\_broadcasting}
    %% }
  }\medskip
  \InEachSynchroRound{$R\in [1..\finalround]$}{\label{line:start:synch:round}

    % #################################### 
    \announceStep{Communication step}
    \broadcast $\msgm(\toBeBcast_{i,R})$
     \Comment*{$p_i$ receives its own broadcast}
    
    \label{line:start:comm:step}\label{line:bcast}
    $\displaystyle\view_i[R]\leftarrow % \view_i[R]\cup
    %    \bigcup_{\substack{\msgm(\setchains_{j,R})\\\in\mathit{received}_{i,R}}} \setchains_{j,R}$
\big\{ \pi\in\setchains_{j,R} \text{, such that } \msgm(\setchains_{j,R})\in\mathit{received}_{i,R} \big\}$\label{line:view:i:R}\;

 %  \Comment*{$p_i$ receives its own broadcast}

    $\displaystyle\toBeBcast_{i,R+1}\leftarrow\{\pi \cryptchain p_i \,|\, \pi\in \view_i[R]\wedge p_i\not\in\pi \}$\label{line:signing:next:round}\label{line:end:comm:step}\;

   % #################################### 
   \announceStep{Computation step}
  
   \lIf{$\ready_i$}{\label{start:computation:step}%
%      $\brbdeliver(\messageToDeliver)$\label{line:brdeliver:ready} ;
      \stopKW\label{line:stop:ready}
    }
    $\knownmessages_{i,R} \leftarrow \messageOf\left(\bigcup_{r\in[1..R]} \view_i[r]\right)$\label{line:computing:knownmsg}\;
    
    \uIf{$R=\finalround$\label{line:reached:finalround}}{
      $W_i \leftarrow \big\{w\in\mathbb{N}\,\big|\,\exists m\in\knownmessages_{i,\finalround}: \certificate_i(m,w)\big\}$\label{line:Wi:set} ;
      \label{line:no:delivery}\lIf{$W_i=\emptyset$}{\stopKW\hspace{-2em}}
      $\wmax{i}\leftarrow \maxfn \left(W_i \right)$\label{line:wmaxj:computed}\;
      $\candidatemsg_i \leftarrow \big\{m\in \knownmessages_{i,\finalround} \,\big|\, \certificate_i(m,\wmax{i}) \big\}$\;
      $\brbdeliver\big(\choice(\candidatemsg_i)\big)$\label{line:brdeliver:finalround}
%      \stopKW%
    }
    \ElseIf{$\knownmessages_{i,R} =\{m\}\:\wedge\: \certificate_i(m,t+3-R)$\label{line:test:knowmessage}}{
      %      $\ready_i \leftarrow \ttrue$ ; $\messageToDeliver\leftarrow m$\label{end:computation:step}\;
      $\brbdeliver(m)$\label{line:brdeliver:immediate} ;
      $\ready_i \leftarrow \ttrue$
      \;
    }\label{end:computation:step}
  }
  \label{line:end:synch:round}
  \caption{Certificate-based Synchronous BRB code for $p_i\neq p_{\orig}$}
  \label{algo:SBRB:pi}
\end{algorithm}

\begin{algorithm}[ht]
  \small
  %% \Fn{$\weight_i(m,X)$}{
  %%   $X_{m,i} = \left\{q\in X\; \left| \;m\cryptchain p_{\orig}\cryptchain q \in \subchain_2\left(\bigcup_{r'\in[1..\finalround]} \view_i[r']\right)\right.\right\}$\;
  %%   \KwRet $|X_{m,i}|$
  %% }\medskip

  %% \Fn{$\braidedwitness_i(m,w,\rmwi,\sequencei)$}{
  %%   \KwRet %\begin{aligned}[t]
  %%     % & % \exists E_1 \subseteq \Pi\setminus\{p_i\},
  %%   $m\cryptchain p_{\orig}\cryptchain \sequencei \cryptchain p_i \in \view_i[\rmwi] \;\wedge$\label{line:chain:ending:w:pi}\;
  %%       % \{m\cryptchain p_{\orig}\cryptchain q \cryptchain \sequencei \,|\, q\in E_1\}&\subseteq \view_i[\rmwi] \;\wedge\\
  %%   \hspace{\widthof{\KwRet}} $\big|\big\{q\in\Pi\setminus\{p_i\}\,\big|\, m\cryptchain p_{\orig}\cryptchain q \cryptchain \sequencei \in \view_i[\rmwi] \big\}\big| \geq \minfn\big(w-2,t+1-\rmwi\big).$\label{line:braids:threshold}\;
  %%   % \end{aligned}
  %%   % \end{aligned}$\label{line:exists:r}
  %% }\medskip

  
  \Fn{$\certificate_i(m,w)$}{
    $S_{i,R}\leftarrow\left\{q\in\Pi\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \subchain_2\left(\bigcup_{r'\in[2..\finalround]} \view_i[r']\right)\right.\right\}$\label{line:S:i:R}\;
    \return $\exists \rmwi\in[2..\finalround], \exists \sequencei \in
%    (\Pi\setminus\{p_i\})^{\rmwi-1}:$\label{line:exist:ri:omegai}\;
    \Pi^{\rmwi-1}:$\label{line:exist:ri:omegai}
    $\begin{cases}
      m\cryptchain p_{\orig}\cryptchain \sequencei \in \view_i[\rmwi]\: \wedge\\
      \left|S_{i,R}\setminus \subchain_{t+2-w}(\sequencei)\right|\geq w-2
    \end{cases}$
    \label{line:chain:ending:w:pi}\label{line:certif:threshold}\;
    % \end{aligned}$\label{line:exists:r}
  }
  \caption{Certificate function}\label{algo:certificate}
\end{algorithm}



==> alg/sync_sig_brb_ta_generic.tex <==
\begin{algorithm}[tb]
  \small
  \InSynchroRound{$R=1$}{
    $\broadcast(\msgm(\{m\cryptchain p_{\orig}\}))$\; \label{line:generic:porig:bcast}
    $\brbdeliver(m)$\; \label{line:generic:porig:brdeliver}
  }
  \caption{\brb-broadcast operation executed by $p_\orig$ at round $R=1$}
  \label{alg:generic:porig:code}
\end{algorithm}

\begin{algorithm}[tb]
\small
\InitStep{$\view_i[1..t{+}1] \gets [\emptyset,...,\emptyset]$;
$\ready_i \gets \ffalse$;
$\toBeBcast_i \gets \emptyset$%
\label{line:generic:viewi:modif}}{}\medskip

\InEachSynchroRound{$R\in [1..\finalround]$}{\label{line:generic:start:synch:round}

    % #################################### 
    \commStep
    
    \lIf{$R \geq 2$}{\broadcast $\msgm(\toBeBcast_i)$} \label{line:generic:bcast} \label{line:generic:start:comm:step}
    \lIf{$\ready_i$}{\stopKW} \label{line:generic:stop:ready} \label{line:generic:end:comm:step}
    
    % ####################################

    
    \compStep
    
    $\view_i[R] \gets \{\pi \in \setchains \mid \msgm(\setchains) \in \received_{i,R}\}$\; \label{line:generic:view:i:R} \label{start:generic:computation:step}
    
    $\toBeBcast_i \gets \{\pi \cryptchain p_i \mid \pi \in \view_i[R] \land p_i \not\in \pi \}$\; \label{line:generic:signing:next:round}
    
    $\knownmessages_{i,R} \gets \messageOf\left(\bigcup_{r\in[1..R]} \view_i[r]\right)$\; \label{line:generic:computing:knownmsg}
    

    \uIf{$\knownmessages_{i,R} = \{m\} \land \exists w\in\mathbb{N}^{+}: \ovalbox{$\delpredicate(m,w,view_i)$} \land \big(R\geq \ovalbox{$\reveal(w)$}\big)$}{ \label{line:generic:test:knowmessage}
      $\brbdeliver(m)$;
      $\ready_i \gets \ttrue$\; \label{line:generic:brdeliver:immediate}
    }
    \ElseIf{$R=\finalround$}{
        \label{line:generic:reached:finalround}
        $\weights_i \gets \{w \in \mathbb{N}^{+} \mid \Exists m \in \knownmessages_{i,R}: \ovalbox{$\delpredicate(m,w,\view_i)$}\}$\;
        \label{line:generic:no:delivery}\label{line:generic:Wi:set}
        
        \If{$\weights_i \neq \emptyset$}{
            $\candidatemsg_i \gets \{m \in \knownmessages_{i,R} \mid \ovalbox{$\delpredicate\big(m,\maxfn(W_i),\view_i\big)$}\}$\;
        
            $\brbdeliver(\choice(\candidatemsg_i))$\; \label{line:generic:brdeliver:finalround}
        }
    }
    \label{end:generic:computation:step}
}
\label{line:generic:end:synch:round}
\caption{Skeleton of a Weight-based Synchronous BRB algorithm (code for $p_i\neq p_{\orig}$). The use of $\delpredicate()$ and $\reveal()$ are highlighted using rounded boxes.}
\label{algo:generic:SBRB:pi}
\end{algorithm}




==> fig/tikz_callouts_pointer_shift.tex <==
\makeatletter

\newlength{\callout@move@pointer@start@x}
\newlength{\callout@move@pointer@start@y}
\pgfkeys{/pgf/.cd,
    callout pointer xshift/.code={\setlength{\callout@move@pointer@start@x}{#1}},
    callout pointer yshift/.code={\setlength{\callout@move@pointer@start@y}{#1}},
}

% \pgf@lib@rectanglecallout@pointer
%
% Internal macro for calculations relating to the rectangle callout.
%
% Requires the following to be set up:
%
% \calloutpointer - the location of the callout point.
% \xtemp          - the half width of the rectangle
% \ytemp          - the half height of the rectangle
% \pointerwidth   - the width of the pointer.
%
\def\pgf@lib@rectanglecallout@pointer{%
    %
    % Ensure that the pointer never connects to the main shape
    % too near to a corner. This is done for two reasons:
    % 1. It can look ugly.
    % 2. If the corners are rounded, a mess can result.
    %
    \pgfextract@process\borderpoint{%
            \pgfpointborderrectangle{%
                \centerpoint%
                \pgf@xa\pgf@x%
                \pgf@ya\pgf@y%
                \calloutpointer%
                \advance\pgf@x-\pgf@xa%
                \advance\pgf@y-\pgf@ya%
            }{\pgfqpoint{\xtemp}{\ytemp}}%
        }%
    \pgfmathanglebetweenpoints{\pgfpointorigin}{\borderpoint}%
    \let\borderangle\pgfmathresult%
    %
    \pgfutil@tempdima\pointerwidth\relax%
    \pgf@xa\xtemp\relax%
    \advance\pgf@xa-\pgfutil@tempdima%
    \pgf@ya\ytemp\relax%
    \advance\pgf@ya-\pgfutil@tempdima%
    %
    \pgf@process{%
        \pgfutil@ifundefined{pgf@corner@arc}{\pgfpointorigin}{%
            \expandafter\pgfqpoint\pgf@corner@arc}%
    }%
    \advance\pgf@xa-\pgf@x%
    \advance\pgf@ya-\pgf@y%
    %
    \borderpoint%
    \pgf@xb\pgf@x%
    \pgf@yb\pgf@y%
    %
    \pgf@xc0pt\relax%
    \pgf@yc0pt\relax%
    %
    \pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{\xtemp}{\ytemp}}%
    \ifdim\borderangle pt<\pgfmathresult pt\relax%
        \pgf@yc.5\pgfutil@tempdima%
        \ifdim\pgf@yb>\pgf@ya%
            \pgf@yb\pgf@ya%
        \fi%
        %
        % Establish the order for drawing the rectangle corners.
        %
        \edef\firstpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
        \edef\secondpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
        \edef\thirdpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
        \edef\fourthpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
    \else%
        \pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{-\xtemp}{\ytemp}}%
        \ifdim\borderangle pt<\pgfmathresult pt\relax%
            \pgf@xc-.5\pgfutil@tempdima%
            \ifdim\pgf@xb>\pgf@xa%
                \pgf@xb\pgf@xa%
            \else%
                \ifdim\pgf@xb<-\pgf@xa%
                    \pgf@xb-\pgf@xa%
                \fi%
            \fi%
            \edef\firstpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
            \edef\secondpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
            \edef\thirdpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
            \edef\fourthpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
        \else%
            \pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{-\xtemp}{-\ytemp}}%
            \ifdim\borderangle pt<\pgfmathresult pt\relax%
                \pgf@yc-.5\pgfutil@tempdima%
                \ifdim\pgf@yb>\pgf@ya%
                    \pgf@yb\pgf@ya%
                \else%
                    \ifdim\pgf@yb<-\pgf@ya%
                        \pgf@yb-\pgf@ya%
                    \fi%
                \fi%
                \edef\firstpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
                \edef\secondpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
                \edef\thirdpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
                \edef\fourthpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
            \else%
                \pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{\xtemp}{-\ytemp}}%
                \ifdim\borderangle pt<\pgfmathresult pt\relax%
                    \pgf@xc.5\pgfutil@tempdima%
                    \ifdim\pgf@xb>\pgf@xa%
                        \pgf@xb\pgf@xa%
                    \else%
                        \ifdim\pgf@xb<-\pgf@xa%
                            \pgf@xb-\pgf@xa%
                        \fi%
                    \fi%
                    \edef\firstpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
                    \edef\secondpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
                    \edef\thirdpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
                    \edef\fourthpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
                \else%
                    \pgf@yc.5\pgfutil@tempdima%
                    \ifdim\pgf@yb<-\pgf@ya%
                        \pgf@yb-\pgf@ya%
                    \fi%
                    \edef\firstpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
                    \edef\secondpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
                    \edef\thirdpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
                    \edef\fourthpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
                \fi%
            \fi%
        \fi%
    \fi%
    \pgfextract@process\beforecalloutpointer{%
        \centerpoint%
        \advance\pgf@x\pgf@xb%
        \advance\pgf@x\callout@move@pointer@start@x% <------------------ ADDED HERE
        \advance\pgf@y\pgf@yb%
        \advance\pgf@y\callout@move@pointer@start@y% <------------------ ADDED HERE
        \advance\pgf@x-\pgf@xc%     
        \advance\pgf@y-\pgf@yc%
    }%  
    \pgfextract@process\aftercalloutpointer{%
        \centerpoint%
        \advance\pgf@x\pgf@xb%
        \advance\pgf@x\callout@move@pointer@start@x% <------------------ ADDED HERE
        \advance\pgf@y\pgf@yb%
        \advance\pgf@y\callout@move@pointer@start@y% <------------------ ADDED HERE
        \advance\pgf@x\pgf@xc%      
        \advance\pgf@y\pgf@yc%
    }%  
    %
    % Now calculate the pointer anchor.
    %
    \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@x>\pgf@y%
        \edef\outersep{\the\pgf@x}%
    \else%
        \edef\outersep{\the\pgf@y}%
    \fi%
    \pgf@lib@callouts@pointeranchor%
}

\makeatother

==> sec/deleted.tex <==

\begin{restatable}[Certificate Conspicuity]{lemma}{lemmaCertificateImpliesMKnown}\label{lemma:certificate:implies:m:known}
  %% If $p_i$ and $p_j$ are correct processes, $m$ is a message, and $R\in [2..\finalround]$ is a round; if $m\not\in\knownmessages_{i,R}$ at round $R$ at line~\ref{line:test:knowmessage} of Algorithm~\ref{algo:SBRB:pi}, then %% for all rounds $R'\in [1..\finalround]$, 
  %% $\certificate_j(m,t+3-R)=\ffalse$ during all of $p_j$'s execution.
  Let $p_i$ and $p_j\neq p_i$ be  correct processes, $m$  a message, and $R\in [2..\finalround]$  a round. 
  If $p_i $ observes a certificate of weight at least $t+3-R$ for $m$ at some point of its execution (i.e.  $\certificate_i(m,t+3-R)=\ttrue$) and  $p_j$ executes round $R$, then $m\in\knownmessages_{j,R}$ at round $R$ at $p_j$.
\end{restatable}

\begin{proofoverview}
  Let us note $\rmwi$ and $\sequencei$ a round and a process sequence that render true the condition at line~\ref{line:chain:ending:w:pi}
  in the  definition of $\certificate_i$ for $p_i$ (Alg.~\ref{algo:certificate}). The proof depends on whether $\rmwi$ (the round in which $p_i$ observes the revealing chain $m\cryptchain p_{\orig}\cryptchain \sequencei$, cf. Alg.~\ref{algo:certificate}) occurs before or after the round $R$, the round during which we seek to prove that all correct processes are aware of $m$.
  If $\rmwi<R$, because $p_i$ forwards all chains it has not signed yet, all correct processes observe a chain containing $m$ at the latest by round $\rmwi+1\leq R$.
  If $\rmwi\geq R$, the fact that only the first process of $\subchain_{t+2-w}(\sequencei)$ can be backing $m$ in $p_i$'s certificate implies that $(t+2-w)+(w-2)+1=t+1$ processes (counting the $(t+2-w)$-prefix of $\sequencei$, the remaining processes of $S_{i,R}$ not in the prefix, and $p_\orig$) have signed a chain containing $m$ during the first $R$ rounds of the protocol. One of them must be correct, yielding the lemma.
\end{proofoverview}

%\lemmaCertificateImpliesMKnown*

\begin{detailedproof}
  Assume a correct process $p_i$ observes 
  $\certificate_i(m,t+3-R)=\ttrue$.
  In the following, $\rmwi$ and $\sequencei$ denote a round and a process sequence that render true the condition at line~\ref{line:chain:ending:w:pi}
   in the  definition of $\certificate_i$ (Algorithm~\ref{algo:certificate}).
   The remainder of the proof distinguishes two cases, depending on whether $\rmwi< R$ or not.
  \begin{itemize}
  \item Case $\rmwi< R$: $m\cryptchain p_{\orig}\cryptchain \sequencei \in \view_i[\rmwi]$ implies that $p_i$ receives $m\cryptchain p_{\orig}\cryptchain \sequencei$ during the communication step of round $\rmwi < R$ (line~\ref{line:view:i:R} of Algorithm~\ref{algo:SBRB:pi}). If $p_i\not\in\sequencei$, $p_i$ signs the chain (line~\ref{line:signing:next:round}, Alg.~\ref{algo:SBRB:pi}), and broadcast it during the communication step of round $\rmwi+1 \leq R$ (line~\ref{line:bcast} of the same algorithm). If $p_i\in\sequencei$, $p_i$ has signed a chain $m\cryptchain p_{\orig}\cryptchain \seq'$ earlier, and broadcast the result before or during round $\rmwi$.

    In both cases, this means all other correct processes receive some chain $m\cryptchain p_{\orig}\cryptchain \sequencei' \cryptchain p_i$ either during or before round $R$, and therefore that $m\in\knownmessages_{j,R}$ at round $R$ for all correct processes $p_j$ that execute round $R$.
  \item Case $\rmwi\geq R$:
    Let us note $\seq_{R-1}=\subchain_{R-1}(\sequencei)$. $m\cryptchain p_{\orig}\cryptchain \sequencei \in \view_i[\rmwi]$ at line~\ref{line:chain:ending:w:pi} means that $|\sequencei|=\rmwi-1$. Since by case assumption $\rmwi\geq R$, $|\sequencei|\geq R-1$, and therefore $|\seq_{R-1}|=|\subchain_{R-1}(\sequencei)|=R-1$.

    Let $E$ denote
       $\left\{q\in\Pi\setminus \seq_{R-1}\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \subchain_2\left({\textstyle\bigcup_{r'\in[1..\rmwi]} \view_i[r']}\right)\right.\right\}.$
       
    The condition of line~\ref{line:certif:threshold} implies $|E|\geq t+1-R$. By construction of $E$, $\seq_{R-1}\cap E=\emptyset$. Similarly, because correct processes only accept acyclic signature chains, $p_{\orig}\not\in E$. For the same reason line~\ref{line:chain:ending:w:pi} of Algorithm~\ref{algo:certificate} implies $p_{\orig}\not\in \seq_{R-1}\subseteq \sequencei$.
        $E$, $\seq_{R-1}$, and $\{p_{\orig}\}$ are therefore pair-wise disjoint. We therefore have $|E \cup \seq_{R-1} \cup \{p_{\orig}\}| = |E| + |\seq_{R-1}| + 1 \geq (t+1-R) + (R-1) + 1 = t+1$.
    $E \cup \seq_{R-1} \cup \{p_{\orig}\}$ therefore contains at least one correct process, $p_k$.
    \begin{itemize}
      \item If $p_k=p_{\orig}$, the sender is correct, and all correct processes observe message $m$ during round $1$.
      \item If $p_k\in E$, $p_k$ has signed a chain of length 2 with message $m$ and has broadcast this chain to all processes during round $2$.
      \item Finally, if $p_k\in\seq_{R-1}$, the facts that $\seq_{R-1}=\subchain_{R-1}(\sequencei)$ and $m\cryptchain p_{\orig}\cryptchain \sequencei \in \view_i[\rmwi]$ at line~\ref{line:chain:ending:w:pi} of Alg.~\ref{algo:certificate} imply that $p_k$ has signed a chain with message $m$ and has broadcast this chain to all processes during or before round $R \leq \rmwi$.
    \end{itemize}
    All three cases imply that all correct processes that have not stopped earlier have observed message $m$ at the latest by the end of the communication step of round $R$, i.e., that $m\in\knownmessages_{j,R}$ at line~\ref{line:test:knowmessage} of Algorithm~\ref{algo:SBRB:pi}.\qedhere
  \end{itemize}
\end{detailedproof}

The following corollary from Lemma~\ref{lemma:certificate:implies:m:known} states that if a correct process has not seen a message $m$ by round $R\geq 2$, then no certificate of weight $\geq t+3-R$ will ever exist. % in the system.

\begin{corollary}\label{coro:m:notknown:nocertif}
  Let  $p_i$ and $p_j\neq p_i$ be correct processes, $m$  a message, and $R\in [2..\finalround]$ a round. If $m\not\in\knownmessages_{i,R}$ at round $R$ at line~{\em\ref{line:test:knowmessage}} of Algorithm~{\em\ref{algo:SBRB:pi}} at $p_i$, then for any $R'\geq R$, %% for all rounds $R'\in [1..\finalround]$, 
  $\certificate_j(m,t+3-R')=\ffalse$ during all of $p_j$'s execution.
\end{corollary}

\begin{proof}
  Consider $p_i$ and $p_j$ two correct processes. If $m\not\in\knownmessages_{i,R}$ at round $R$ of $p_i$, then by contrapositive of Lemma~\ref{lemma:certificate:implies:m:known}, then  $\certificate_j(m,t+3-R)=\ffalse$ during all of $p_j$'s execution. Because of the inequality at line~\ref{line:certif:threshold} of the definition \certificate (Alg.~\ref{algo:certificate}), $\certificate_j(m,w)$ implies $\certificate_j(m,w')$ for any $w'\leq w$, and therefore $\certificate_j(m,t+3-R)=\ffalse$ implies $\certificate_j(m,t+3-R')=\ffalse$ for any $R'\geq R$.
\end{proof}

\begin{lemma}[Certificate Final Visibility] \label{lemma:certifi:R:certifj:t+1}
Let $p_{\orig}$ be Byzantine, and $p_i$ and $p_j$ be correct processes such that $p_i$ observes $\certificate_i(m,w)=\ttrue$ at some round $R\in [1..\finalround]$, and $p_j$ executes the communication step of round $\finalround$.
Then $p_j$ observes $\certificate_j(m,w)=\ttrue$ at round $\finalround$.
\end{lemma}

\begin{proof}
Assume a correct process $p_i$ observes $\certificate_i(m,w)=\ttrue$ at some round $R$. Consider $p_j$ another correct process that reaches round $\finalround$. Without loss of generality, assume $p_j\neq p_i$ (as the case $p_i=p_j$ is trivial).

In the following, $\rmwi$ and $\sequencei$ denote a round and a process sequence that render true the condition at line~\ref{line:generic:chain:ending:w:pi} %% -\ref{line:generic:certif:threshold}
for $p_i$ in the  definition of $\certificate_i$ (Algorithm~\ref{algo:certificate}).

Let $E_{i,R}$ be the value of $S_{i,R}\setminus \subchain_{t+2-w}(\sequencei)$ at line~\ref{line:generic:certif:threshold} of Alg.~\ref{algo:certificate} at $p_i$ in round $R$
\begin{equation}\label{eq:def:E:R:i}
E_{i,R}=\textstyle\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencei)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \truncate_2\left(\bigcup_{r'\in[2..\finalround]} \view_i[r']\right)\right.\right\}.
\end{equation}
By lemma assumption, $|E_{i,R}|\geq w-2$. Furthermore, as $\view_i[r']$ is initially empty and only updated during round $r'$, during round $R$,
$%\begin{equation*}
  \forall r'> R: \view_i[r']=\emptyset.
$ %\end{equation*} 
At round $R$, we therefore have
$%\begin{align*}
  \textstyle
\truncate_2\left(\bigcup_{r'\in[2..\finalround]} \view_i[r']\right)
= \textstyle\truncate_2\left(\bigcup_{r'\in[2..R]} \view_i[r']\right) = \accumulatorTwo{i}[R].
 % \\   &= \accumulatorTwo{i}[R].
$ %\end{align*}
We can therefore rewrite (\ref{eq:def:E:R:i}) into
\begin{equation}\label{eq:def:E:R:i:T2}
E_{i,R}=\textstyle\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencei)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{i}[R]\right.\right\}.
\end{equation}

The rest of the proof distinguishes two cases, depending on whether $p_j\in \sequencei$ or not, with the case $p_j\not\in \sequencei$ leading to more sub-cases.
\begin{itemize}
\item Case $p_j\in \sequencei$: As $p_j$ is correct, $p_j\in \sequencei$ implies $p_j$ has signed and therefore received a chain $m\cryptchain p_{\orig} \cryptchain \sequencej$ at line~\ref{line:generic:signing:next:round} of Alg.~\ref{algo:generic:SBRB:pi} during some round $\rmwj<\rmwi$, where $\sequencej$ is a prefix of $\sequencei$.
As a result of this broadcast, at all rounds higher or equal to $\rmwj$, we have
\begin{equation}\label{eq:chain:pj}
    m\cryptchain p_{\orig} \cryptchain \sequencej \in \view_j[\rmwj].
\end{equation}
  
  As $\sequencej$ is a prefix of $\sequencei$, $\subchain_{t+2-w}(\sequencej)$ is also a prefix of $\subchain_{t+2-w}(\sequencei)$, which implies using (\ref{eq:def:E:R:i:T2})
  \begin{align*}
    E_{i,R}&\subseteq \textstyle\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencej)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{i}[R]\right.\right\},\\
    &\subseteq \textstyle\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencej)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{j}[t+1]\right.\right\}\tag*{using Corollary~\ref{coro:T2:i:r:in:T2:j:final}.}
  \end{align*}
  As $|E_{i,R}|\geq w-2$ (since $\certificate_i(m,w)=\ttrue$ at round $R$ by lemma assumption), this last inclusion yields
  \begin{equation}\label{eq:length:2:prefix:pj:geq:wm2}
    \textstyle\left|\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencej)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{j}[t+1]\right.\right\}\right|\geq w-2.
  \end{equation}
  Equations~(\ref{eq:chain:pj}) and (\ref{eq:length:2:prefix:pj:geq:wm2}) render true line~\ref{line:generic:chain:ending:w:pi} %% and~\ref{line:generic:certif:threshold}
  of $\certificate_j(m,w)$ (Alg.~\ref{algo:certificate}) at round $t+1$, proving the lemma.

\item Case $p_j\not\in\sequencei$: If $p_j$'s signature is not in $\sequencei$ the approach to find $\rmwj$ and $\sequencej$ that fulfill line~\ref{line:generic:chain:ending:w:pi} %% -\ref{line:generic:certif:threshold}
  of Alg.~\ref{algo:certificate} for $p_j$ depends on the value of $\rmwi$ and on whether $p_i$ appears in the set $E_{i,R}$ of length-2 prefixes.

  Line~\ref{line:generic:chain:ending:w:pi} of Alg.~\ref{algo:certificate} implies $\view_i[\rmwi]\neq \emptyset$. As $\view_i[\rmwi]$ is initially empty and only updated in the communication step of round $\rmwi$, this implies $R \geq \rmwi$.
  \begin{itemize}
  \item Case $\rmwi=t+1$:
      $R \geq \rmwi$ yields $R\geq t+1$. As $R\leq t+1$ by lemma assumption, we conclude $R=t+1$.
      %\ft{Use earlier lemma on $\accumulatorTwo{i|j}[R]$}
      Since $p_{\orig}\not\in\sequencei$ due to the acyclic nature of signature chains accepted by correct processes, $|\{p_{\orig}\}\cup\sequencei|=|\{p_{\orig}\}|+|\sequencei|=1+\rmwi-1=t+1$ (by case assumption). $\{p_{\orig}\}\cup\sequencei$ therefore contains at least one correct process $p_k$. As $p_{\orig}$ is Byzantine (by lemma assumption), $p_k\in\sequencei$. 
      %% \begin{itemize}
      %% \item If $\sequencei$ contains at least one correct process $p_k$, 
        this means that $p_k$ has broadcast to all processes a chain $m\cryptchain p_{\orig}\cryptchain \sequencej$ during some round $\rmwj\leq t+1$, where $\sequencej$ is a prefix of $\sequencei$. $p_j$ has received this chain, and we therefore have
        \begin{equation}\label{eq:chain:pj:3}
          m\cryptchain p_{\orig}\cryptchain \sequencej \in \view_j[\rmwj].
        \end{equation}
        Furthermore, since $\sequencej$ is a prefix of $\sequencei$, we have
        \begin{align*}
          \hspace{-1em}E_{t+1,i}&\subseteq \textstyle\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencej)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{i}[t+1]\right.\right\},\\
          &\subseteq  \textstyle\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencej)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{j}[t+1]\right.\right\},\tag*{using Lemma~\ref{lemma:T2:equal:final:round}.}
        \end{align*}
        As above, $|E_{t+1,i}|\geq w-2$ (since $R=t+1$, see above) implies that this last set contains at least $w-2$ elements. This fact with (\ref{eq:chain:pj:3}) renders true line~\ref{line:generic:chain:ending:w:pi} %% and~\ref{line:generic:certif:threshold}
        of $\certificate_j(m,w)$ (Alg.~\ref{algo:certificate}) at round $t+1$, proving the lemma.
        %\ft{$p_j$ has seen a prefix of $\sequencei$.}
      %% \item If $\sequencei$ contains no correct process, as $p_{\orig}$ is Byzantine by Lemma assumption, the set $\seq_i=\{p_{\orig}\}\cup\sequencei$ only contains Byzantine processes. Furthermore since $p_{\orig}\not\in\sequencei$ due to the acyclic nature of signature chains, $|\seq_i|=|\{p_{\orig}\}|+|\sequencei|=1+\rmwi-1=t+1$ (by case assumption).
      %%   \ft{All of $E_{i,R}$ must then be correct}
%          \end{itemize}

  \item Case $\rmwi<t+1$:
    \begin{itemize}
    \item Sub-case $p_i\not\in E_{i,R}$ or $|\sequencei|\geq t+2-w$: 
%          
      Line~\ref{line:generic:chain:ending:w:pi} of Alg.~\ref{algo:certificate} implies $m\cryptchain p_{\orig}\cryptchain \sequencei \in \view_i[\rmwi]$. If $p_i\not\in \sequencei$, $p_i$ signs the chain $m\cryptchain p_{\orig}\cryptchain \sequencei$ (line~\ref{line:generic:signing:next:round}, Alg.~\ref{algo:generic:SBRB:pi}) and broadcasts to all processes (since $p_i$ is correct) the chain $m\cryptchain p_{\orig}\cryptchain \sequencei \cryptchain p_i$ during the communication step of round $\rmwi+1$. If $p_i\in \sequencei$, this means $p_i$ has already performed these two steps (signing and broadcasting) at some earlier round.

      In both cases, $p_j$ receives a chain $m\cryptchain p_{\orig}\cryptchain \sequencei' \cryptchain p_i$ during some round $\rmwj\leq\rmwi+1$. By choosing $\sequencej=\sequencei' \cryptchain p_i$, we therefore have
      \begin{equation}\label{eq:chain:pj:2}
        m\cryptchain p_{\orig}\cryptchain \sequencej \in \view_j[\rmwj].
      \end{equation}
      %% By definition of $\sequencej = \sequencei \cryptchain p_i$,
      If $p_i\in \sequencei$, then $\sequencej$ is a prefix of $\sequencei$, $\subchain_{t+2-w}(\sequencej)\subseteq\subchain_{t+2-w}(\sequencei)$ and 
      \begin{align}\label{eq:E:R:i:with:sequencej}
        E_{i,R}\subseteq&\textstyle\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencej)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{i}[R]\right.\right\}.
      \end{align}
      If $p_i\not\in \sequencei$ and $|\sequencei|\geq t+2-w$, then $\sequencei'=\sequencei$,  $\subchain_{t+2-w}(\sequencej)=\subchain_{t+2-w}(\sequencei)$ and (\ref{eq:E:R:i:with:sequencej}) still holds.
      %% \begin{align}\label{eq:E:R:i:with:sequencej}
      %%   E_{i,R}=&\textstyle\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencej)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{i}[R]\right.\right\}.
      %% \end{align}
      Finally if $p_i\not\in \sequencei$ and $|\sequencei|< t+2-w$, then $\sequencei'=\sequencei$, $\subchain_{t+2-w}(\sequencej)$ contains an extra terminal $p_i$ compared to $\subchain_{t+2-w}(\sequencei)$. However, by case assumption $|\sequencei|< t+2-w$ implies $p_i\not\in E_{i,R}$, and therefore (\ref{eq:E:R:i:with:sequencej}) continues to hold.
      %% This implies that $\Pi\setminus \subchain_{t+2-w}(\sequencej)$ differs from $\Pi\setminus \subchain_{t+2-w}(\sequencei)$ by at most $\{p_i\}$ (which might be excluded from the first, while it is present in the second), but as $p_i\not\in E_{i,R}$ by assumption, this does not impact the value of $E_{i,R}$. 
      Using Corollary~\ref{coro:T2:i:r:in:T2:j:final} on (\ref{eq:E:R:i:with:sequencej}) we therefore have independently of $\sequencei$
      \begin{align*}
        E_{i,R}\subseteq&\textstyle\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencej)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{j}[t+1]\right.\right\}.
      \end{align*}
      As above, using $|E_{i,R}|\geq w-2$ on the above inclusion yields
      \begin{equation}\label{eq:length:2:prefix:pj:geq:wm2:2}
        \textstyle\left|\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencej)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{j}[t+1]\right.\right\}\right|\geq w-2.
      \end{equation}
      Equations~(\ref{eq:chain:pj:2}) and (\ref{eq:length:2:prefix:pj:geq:wm2:2}) render true line~\ref{line:generic:chain:ending:w:pi} %% and~\ref{line:generic:certif:threshold}
      of $\certificate_j(m,w)$ (Alg.~\ref{algo:certificate}) at round $t+1$ (since $\rmwj = \rmwi +1 \leq t+1$ by case assumption), proving the lemma.

    \item Sub-case $p_i\in E_{i,R}$ and $|\sequencei|< t+2-w$: 
      %
      $p_i\in E_{i,R}$ means that $p_i$ has signed $m\cryptchain p_{\orig}$. Since $p_i$
      is correct, it has therefore broadcast to all processes $m\cryptchain p_{\orig}\cryptchain p_i$ during round $2$. As a result, from round 2 onward
      \begin{equation}\label{eq:p:i:new:sequencej}
        m\cryptchain p_{\orig}\cryptchain p_i\in \view_j[2].
      \end{equation}

      By definition $\rmwi\geq 2$ (line~\ref{line:generic:exist:ri:omegai} of Alg.~\ref{algo:certificate}), and therefore $|\sequencei|=\rmwi-1\geq 1$, implying $\sequencei$ is non-empty (and $t+2-w>1$ by sub-case assumption). Consider $p_\seq$ the first process in $\sequencei$. As $|\sequencei|< t+2-w$ (sub-case assumption), $p_\seq\in \subchain_{t+2-w}(\sequencei)$, and therefore
%          \begin{equation}\label{eq:p:omega:not:in:E:R:i}
        $p_\seq\not\in E_{i,R},$
%          \end{equation}
      by definition of $E_{i,R}$ (Equations~\ref{eq:def:E:R:i} and \ref{eq:def:E:R:i:T2}).

      %% The first part of the sub-case assumption, $p_i\in E_{i,R}$, further implies that $p_i\not\in \subchain_{t+2-w}(\sequencei)$ (by definition of $E_{i,R}$). The second part of the sub-case assumption, $|\sequencei|< t+2-w$, implies that $\subchain_{t+2-w}(\sequencei)=\sequencei$, and hence with the previous observation that $p_i\not\in\sequencei$. As $p_\seq$ is the first process of $\sequencei$, this yields $p_\seq\neq p_i$, and with (\ref{eq:p:omega:not:in:E:R:i})
      %% \begin{equation}\label{eq:p:omega:not:in:E:R:i:minus:pi}
      %%   p_\seq\not\in E_{i,R}\setminus \{p_i\}.
      %% \end{equation}
      We construct a set of length-2 prefixes for $p_j$ by removing $p_i$ and adding $p_\seq$ from/to $E_{i,R}$. More precisely, we have
      \begin{align}
        \big(E_{i,R}\setminus\{p_i\}\big)\cup\{p_\seq\}\hspace{-5em}\nonumber\\
        =&\textstyle\big(\left\{q\in\Pi\setminus \subchain_{t+2-w}(\sequencei)\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{i}[R]\right.\right\}\setminus\left\{p_i\right\}\big)\cup\{p_\seq\},\nonumber\\
%            
        =&\textstyle\big(\left\{q\in\Pi\setminus\{p_i\}\,
        \left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{i}[R]\right.\right\}\setminus \subchain_{t+2-w}\left(\sequencei\right)\big)\cup\{p_\seq\},\nonumber\\
%           
        \subseteq&\textstyle\left\{q\in\Pi\setminus\{p_i\}\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{i}[R]\right.\right\}\cup\{p_\seq\}.\label{eq:E:R:i:minus:cup}
     \end{align}
     Moreover as $m\cryptchain p_{\orig}\cryptchain \sequencei \in \view_i[\rmwi]$ (line~\ref{line:generic:chain:ending:w:pi} of Alg.~\ref{algo:certificate}), and $R\geq \rmwi$,
%          \begin{equation*}
        $m\cryptchain p_{\orig}\cryptchain p_\seq =$ $\truncate_2(p_{\orig}\cryptchain \sequencei) \in \accumulatorTwo{i}[R].$
%          \end{equation*}
      Because $p_\seq\neq p_i$ (since $p_i\in E_{i,R}$ and $p_\seq\not\in E_{i,R}$), this last statement implies
      $p_\seq\in \left\{q\in\Pi\setminus\{p_i\}\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{i}[R]\right.\right\},$
      which with (\ref{eq:E:R:i:minus:cup}) yields
      \begin{align}
        \hspace{-2em}\big(E_{i,R}\setminus\{p_i\}\big)\cup\{p_\seq\}
        \subseteq&\textstyle\left\{q\in\Pi\setminus\{p_i\}\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{i}[R]\right.\right\},\nonumber\\
        \subseteq&\textstyle\left\{q\in\Pi\setminus\{p_i\}\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{j}[t+1]\right.\right\}\tag*{using Corollary~\ref{coro:T2:i:r:in:T2:j:final}.}\label{eq:E:R:i:minus:cup2}
      \end{align}
      As $p_i\in E_{i,R}$ by case assumption, and $p_\seq\not\in E_{i,R}$, $| \big(E_{i,R}\setminus\{p_i\}\big)\cup\{p_\seq\}|= |E_{i,R}|-1+1=|E_{i,R}|$. As $|E_{i,R}|\geq w-2$ (since $\certificate_i(m,w)=\ttrue$ at round $R$ by lemma assumption), the above inclusion leads to
      \begin{equation}\label{eq:E:R:i:minus:plus:larger}
        \hspace{-5em}\big|\textstyle\left\{q\in\Pi\setminus\{p_i\}\,\left|\, m\cryptchain p_{\orig}\cryptchain q \in \accumulatorTwo{j}[t+1]\right.\right\}\big|
        \geq \big|\big(E_{i,R}\setminus\{p_i\}\big)\cup\{p_\seq\}\big|
        = |E_{i,R}|
        \geq w-2.
      \end{equation}
      By choosing $\sequencej=p_i$ and $\rmwj=2$, (\ref{eq:p:i:new:sequencej}) and (\ref{eq:E:R:i:minus:plus:larger}) render true line~\ref{line:generic:chain:ending:w:pi} %% and~\ref{line:generic:certif:threshold}
      of $\certificate_j(m,w)$ (Alg.~\ref{algo:certificate}) at round $t+1$ (since $t\geq 1$, and $t+1\geq 2$), proving the lemma.
    \end{itemize}
  \end{itemize}
\end{itemize}\vspace{-\baselineskip}%
\end{proof}


\subsection{Proof of Theorem~\ref{theo:algo:SBRB:works}}

\begin{proofsketch}
  \begin{itemize}
  \item \brbVprop follows from the use of (secure) signatures and the fact that correct processes only accept valid signature chains.
  
  \item \brbNDNprop is ensured by construction of the algorithm, and \brbLDprop from the code executed by $\psender$ when it is correct.
  
  \item \brbNDYprop follows from \brbVprop when $\psender$ is correct. When $\psender$ is Byzantine,  the no-duplicity follows from the Conspicuity of the certificates (Lemma~\ref{lemma:certificate:implies:m:known}) and %% , if at least one of the processes \brb-delivers in the final round $t+1$,
    from their Final Visibility (Lemma~\ref{lemma:certifi:R:certifj:t+1}).

  Certificate conspicuity ensures that if two processes $p_i$ and $p_j$ \brb-deliver a message before round $t+1$, the process with the ``weaker'' certificate (say $p_j$) must be aware of $p_i$'s message when it \brb-delivers its own message, and therefore must \brb-deliver the same message as $p_i$, due to the condition at line~\ref{line:generic:brdeliver:immediate}.

  If $p_i$ \brb-delivers before round $t+1$ and $p_j$ during round $t+1$, then the Final Visibility of certificates guarantees that $p_j$ will observe $p_i$'s certificate at line~\ref{line:generic:Wi:set}. Corollary~\ref{coro:m:notknown:nocertif} implies that $p_i$'s message is guaranteed to have the ``heaviest'' certificate, ensuring agreement.

  Finally, if both $p_i$ and $p_j$ deliver in round $t+1$, Final Visibility guarantees they see the same set of messages and certificates and that they \brb-deliver the same message.
  % three different cases must be considered, depending on whether the two correct processes \brb-deliver their message before round $t+1$ or during round $t+1$.
  
  \item The good-case latency of the algorithm, $\maxfn(2,t+3-c)$ rounds, follow from the observation that all correct processes observe a certificate of weight $c$ by the end of round $2$ when the initial sender, $\psender$, is correct. As no other message exists in the system, the condition at line~\ref{line:generic:test:knowmessage} ensures that all correct processes have delivered $\psender$'s message at the latest either by the end of round $2$ or by the end of round $t+3-c$, whichever occurs first.

  \item \brbGDprop follows from the above reasoning 
  % on the good-case latency 
  when $\psender$ is correct. When $\psender$ is Byzantine, %the property arises from the following observation:
  the property follows from Certificate Finality.

%  if a correct process $p_i$ \brb-delivers a message $m$, this message is necessarily backed by a certificate of at least a weight $w=2$ (since $\psender$ and another process, possibly $p_i$, must have signed a chain containing $m$ by the end of round $2$). By Certificate Finality, all remaining processes will therefore observe $m$ at the latest by round $t+1$, and \brb-deliver some message.
  \end{itemize}\vspace{-\baselineskip}%
\end{proofsketch}
% \subsubsection{Proof of Theorem~\ref{theo:algo:SBRB:works}}

\ft{The following does no longer fit here, but can probably be used somewhere else.}
\revise{
Theorem~\ref{theo:algo:SBRB:works} hinges on two fundamental properties: \emph{Predicate Conspicuity} (Lemma~\ref{lemma:GCL:predicate:implies:m:known}) and \emph{Certificate Final Visibility} (Lemma~\ref{lemma:certifi:R:certifj:t+1}). Lemmas~\ref{lemma:accum:i:R:in:j:RpOne}-\ref{lemma:T2:equal:final:round} are used to prove Lemma~\ref{lemma:certifi:R:certifj:t+1}.
}
\revise{
As explained earlier, \emph{Certificate Conspicuity} forces Byzantine processes that seek to hide a certificate of weight $w$ for a message $m$ to reveal at the latest by round $t+3-w$ (the ``revealing round'' of $w$) that $m$ exists. \emph{Certificate Final Visibility} ensures that when the initial sender $\psender$ is malicious, if a correct process reaches round $t+1$, %without having \brb-delivered any message,
then this correct process observes all the certificates ever observed by other correct processes. % at some point of their execution.
}


\ft{The following should probably go in an earlier section.}
\revise{
In terms of vocabulary, we say that $p_i$ \emph{observes a predicate} of weight $w$ for a message $m$ during round $R$ if $\GCLpredicate_i(m,w)=\ttrue$ during the computation step of round $R$ at $p_i$ (lines~\ref{start:computation:step}-\ref{end:computation:step} of Algorithm~\ref{algo:SBRB:pi}).
Note that because $\view_i[R]$ is initially empty and is only modified once (during round $R$, line~\ref{line:viewi:modif} of Algorithm~\ref{algo:SBRB:pi}), $\GCLpredicate_i(m,w)$ is stable (once \ttrue during some round, $\GCLpredicate_i(m,w)$ remains true in all subsequent rounds).
For the same reasons, and by definition of $\GCLpredicate_i$ (Algorithm~\ref{algo:GCL:predicate}), if $\GCLpredicate_i(m,w)=\ttrue$ for some weight $w$, then $\GCLpredicate_i(m,w')=\ttrue$ for any smaller weight $w' \leq w$.
}

\ft{Explanation that should probably go into Section~\ref{sec:fram-constr-determ}}
\revise{The following lemma states that if $p_{\orig}$ behaves maliciously (for instance, by sending different messages in round 1), if a certificate of weight $w$ exists for a message $m$ (meaning that it is observed at some point by some correct process), then all correct processes that reach round $\finalround$ observe a certificate of weight $w$ for $m$ by round $\finalround$, a property we have dubbed \emph{Final Certificate Visibility}.}


